Uniform Generation of Temporal Graphs with Given Degrees

Uniform sampling from the set $\mathcal{G}(\mathbf{d})$ of graphs with a given degree-sequence $\mathbf{d} = (d_1, \dots, d_n) \in \mathbb N^n$ is a classical problem in the study of random graphs. We consider an analogue for temporal graphs in which the edges are labeled with integer timestamps. The input to this generation problem is a tuple $\mathbf{D} = (\mathbf{d}, T) \in \mathbb N^n \times \mathbb N_{>0}$ and the task is to output a uniform random sample from the set $\mathcal{G}(\mathbf{D})$ of temporal graphs with degree-sequence $\mathbf{d}$ and timestamps in the interval $[1, T]$. By allowing repeated edges with distinct timestamps, $\mathcal{G}(\mathbf{D})$ can be non-empty even if $\mathcal{G}(\mathbf{d})$ is, and as a consequence, existing algorithms are difficult to apply. We describe an algorithm for this generation problem which runs in expected time $O(M)$ if $\Delta^{2+\epsilon} = O(M)$ for some constant $\epsilon > 0$ and $T - \Delta = \Omega(T)$ where $M = \sum_i d_i$ and $\Delta = \max_i d_i$. Our algorithm applies the switching method of McKay and Wormald $[1]$ to temporal graphs: we first generate a random temporal multigraph and then remove self-loops and duplicated edges with switching operations which rewire the edges in a degree-preserving manner.

==> figures/d_switching.tex <==
\def\node#1{}
\def\thickness{thick}
\def\saturation{15}
\begin{tikzpicture}[
	point/.style={
		draw,
		circle,
		inner sep=0,
		fill,
		minimum width=0.35em,
		minimum height=0.35em
	},
	vertex/.style={
		draw,
		circle,
		inner sep=0.25em,
		\thickness
	},
	edge/.style={
		draw, 
		black, 
		solid,
		\thickness
	}]
	
	%\filldraw[fill=red!\saturation!white, draw=black!0!black, \thickness, rounded corners] (-5.25em,5.5em) rectangle (-0.75em,1em);
	\node (t1) at (-4.5em, 5em) {\footnotesize{$t_1$}};
	\node[vertex] (1v1) at (-3em, 2.5em) {$v_1$};
	\draw[edge] (-3.75em, 3em) .. controls (-5em, 5.5em) and (-1.0em, 5.5em) .. (-2.25em, 3em);
	
	%\filldraw[fill=green!\saturation!white, draw=black!0!black, \thickness, rounded corners] (-7.5em,0em) rectangle (-3.5em,-6em);
	\node (t2) at (-6.25em, -2.75em) {\footnotesize{$t_2$}};
	\node[vertex] (1v2) at (-5.5em, -1em) {$v_2$};
	\node[vertex] (1v4) at (-5.5em, -4.5em) {$v_4$};
	\path[edge] (1v2) -- (1v4);
	
	%\filldraw[fill=green!\saturation!white, draw=black!0!black, \thickness, rounded corners] (-2.5em,0em) rectangle (1.5em,-6em);
	\node (t3) at (-1.25em, -2.75em) {\footnotesize{$t_3$}};
	\node[vertex] (1v3) at (-0.5em, -1em) {$v_3$};
	\node[vertex] (1v5) at (-0.5em, -4.5em) {$v_5$};
	\path[edge] (1v3) -- (1v5);
	
	\path[->, thick, draw] (3.5em,  -0.25em) -- (6.5em,  -0.25em) {};
	
	%\filldraw[fill=green!\saturation!white, draw=black!0!black, \thickness, rounded corners] (8.5em,5.5em) rectangle (12.5em,-2em);
	\node (t4) at (11.25em, 1.25em) {\footnotesize{$t_4$}};
	\node[vertex] (2v1) at (13em, 2.5em) {$v_1$};
	\node[vertex] (2v2) at (10.5em, -1em) {$v_2$};
	\path[edge] (2v1) -- (2v2);
	
	%\filldraw[fill=green!\saturation!white, draw=black!0!black, \thickness, rounded corners] (13.5em,5.5em) rectangle (17.5em,-2em);
	\node (t5) at (14.75em, 1.25em) {\footnotesize{$t_5$}};
	\node[vertex] (2v3) at (15.5em, -1em) {$v_3$};
	\path[edge] (2v1) -- (2v3);
	
	%\filldraw[fill=green!\saturation!white, draw=black!0!black, \thickness, rounded corners] (8.5em,-3em) rectangle (17.5em,-6em);
	\node (t6) at (13em, -3.75em) {\footnotesize{$t_6$}};
	\node[vertex] (2v4) at (10.5em, -4.5em) {$v_4$};
	\node[vertex] (2v5) at (15.5em, -4.5em) {$v_5$};
	\path[edge] (2v4) -- (2v5);
\end{tikzpicture}

==> figures/tcm-outputs.tex <==
\def\node#1{}
\def\thickness{thick}
\def\saturation{15}
\begin{tikzpicture}[
	point/.style={
		draw,
		circle,
		inner sep=0,
		fill,
		minimum width=0.35em,
		minimum height=0.35em
	},
	vertex/.style={
		draw,
		circle,
		inner sep=0.25em,
		\thickness,
		fill=white
	},
	edge/.style={
		draw, 
		black, 
		solid,
		\thickness
	}]
	
	%\node (t1) at (-12em, 3em) {\Large $t=1$};
	%\node (t2) at (-12em, -7em) {\Large $t=2$};
	
	\node (G1) at (-1.5em, 9em) {\Large $G_1$};
	
	\filldraw[fill=green!\saturation!white, draw=black!0!black, \thickness, rounded corners] (-6em, 7.5em) rectangle (3em, -1.5em);
	\node (t1) at (-4.75em, 7em) {\footnotesize{$t=1$}};
	\node[vertex] (11v1) at (-4em, 5em) {$v_1$};
	\node[vertex] (11v2) at (1em, 5em) {$v_2$};
	\node[vertex] (11v3) at (-4em, 1em) {$v_3$};
	\node[vertex] (11v4) at (1em, 1em) {$v_4$};
	\path[edge] (11v1) -- (11v2);
	\path[edge] (11v3) -- (11v4);
	
	\filldraw[fill=green!\saturation!white, draw=black!0!black, \thickness, rounded corners] (-6em, -2.5em) rectangle (3em, -11.5em);
	\node (t1) at (-4.75em, -3em) {\footnotesize{$t=2$}};
	\node[vertex] (12v1) at (-4em, -5em) {$v_1$};
	\node[vertex] (12v2) at (1em, -5em) {$v_2$};
	\node[vertex] (12v3) at (-4em, -9em) {$v_3$};
	\node[vertex] (12v4) at (1em, -9em) {$v_4$};
	\path[edge] (12v1) -- (12v3);
	\path[edge] (12v2) -- (12v4);
	
	\path[thick, draw] (6em,  10em) -- (6em,  -13em) {};
	
	\node (G2) at (13.5em, 9em) {\Large $G_2$};
	
	\filldraw[fill=green!\saturation!white, draw=black!0!black, \thickness, rounded corners] (9em, 7.5em) rectangle (18em, -1.5em);
	\node (t1) at (10.25em, 7em) {\footnotesize{$t=1$}};
	\node[vertex] (21v1) at (11em, 5em) {$v_1$};
	\node[vertex] (21v2) at (16em, 5em) {$v_2$};
	\node[vertex] (21v3) at (11em, 1em) {$v_3$};
	\node[vertex] (21v4) at (16em, 1em) {$v_4$};
	\path[edge] (21v1) -- (21v2);
	\path[edge] (21v3) -- (21v4);
	
	\filldraw[fill=green!\saturation!white, draw=black!0!black, \thickness, rounded corners] (9em, -2.5em) rectangle (18em, -11.5em);
	\node (t1) at (10.25em, -3em) {\footnotesize{$t=2$}};
	\node[vertex] (22v1) at (11em, -5em) {$v_1$};
	\node[vertex] (22v2) at (16em, -5em) {$v_2$};
	\node[vertex] (22v3) at (11em, -9em) {$v_3$};
	\node[vertex] (22v4) at (16em, -9em) {$v_4$};
	\path[edge] (22v1) -- (22v2);
	\path[edge] (22v3) -- (22v4);
	
	\path[thick, draw] (21em,  10em) -- (21em,  -13em) {};
	
	\node (G3) at (28.5em, 9em) {\Large $G_3$};
	
	\filldraw[fill=red!\saturation!white, draw=black!0!black, \thickness, rounded corners] (24em, 7.5em) rectangle (33em, -1.5em);
	\node (t1) at (25.25em, 7em) {\footnotesize{$t=1$}};
	\node[vertex] (31v1) at (26em, 5em) {$v_1$};
	\node[vertex] (31v2) at (31em, 5em) {$v_2$};
	\node[vertex] (31v3) at (26em, 1em) {$v_3$};
	\node[vertex] (31v4) at (31em, 1em) {$v_4$};
	\draw[edge] (31v1) to[bend right] (31v2);
	\draw[edge] (31v1) to[bend left] (31v2);
	\path[edge] (31v3) -- (31v4);
	
	\filldraw[fill=green!\saturation!white, draw=black!0!black, \thickness, rounded corners] (24em, -2.5em) rectangle (33em, -11.5em);
	\node (t1) at (25.25em, -3em) {\footnotesize{$t=2$}};
	\node[vertex] (32v1) at (26em, -5em) {$v_1$};
	\node[vertex] (32v2) at (31em, -5em) {$v_2$};
	\node[vertex] (32v3) at (26em, -9em) {$v_3$};
	\node[vertex] (32v4) at (31em, -9em) {$v_4$};
	\path[edge] (32v3) -- (32v4);
\end{tikzpicture}

==> preliminaries.tex <==
A common definition of a temporal graph is as follows.
\begin{definition}[Temporal (Multi-)Graph]
A temporal (multi-)graph $G = (V, E)$ consists of a set of nodes $V = \{v_1, \dots, v_n\}$ and a (multi-)set of temporal edges $E = \{e_1, \dots, e_m\}$ where each temporal edge is a tuple $(\{u, v\}, t) \in \{ \{u, v\} | u, v \in V \} \times \mathbb N_{>0}$.
The presence of an edge $(\{u, v\}, t)$ in the edge set $E$ indicates that the nodes $u$ and $v$ are connected at time $t$.
To access the node set and timestamp of an edge individually, we define the functions $\sigma((\{u, v\}, t)) = \{u, v\}$ and $\tau((\{u, v\}, t)) = t$, and to access the set of edges without timestamps, we define $\Sigma(E) = \{ \sigma(e) : e \in E \}$.
\end{definition}

\noindent
An important notion to our purpose is that of \emph{simplicity} of an edge or graph.
Given a node set $\sigma(e) = \{v_i, v_j\}$ where $v_i, v_j \in V$, consider the maximal (multi-)subset $R \subseteq \Sigma(E)$ such that $\sigma(e') = \sigma(e)$ for all $\sigma(e') \in R$, i.e. where the edges share the same node set.
Then, we define $m_{i,j} := |R|$ and call $m = m_{i,j}$ the \emph{multiplicity} of the edge $e$.
Note that if $\sigma(e) \notin \Sigma(E)$, then $R = \emptyset$ and $m_{i,j} = 0$.
On the other hand, if $m \geq 2$, then we say that $e$ is contained in an (ordinary) \emph{multi-edge}, and in the special cases $m = 2$ or $m = 3$, we refer to the multi-edge as a \emph{double-edge} or \emph{triple-edge}, respectively.
As a counterpart to ordinary multi-edges, we also define \emph{temporal} multi-edges as follows.
Again, consider the maximal (multi-)subset $S \subseteq E$ such that $e' = e$ for all $e' \in S$, i.e. where the edges share both the same node set and the same timestamp.
Then, we define $w_{i,j,t} := |S|$, call $w = w_{i,j,t}$ the \emph{temporal multiplicity} of the edge $e$, and if $w \geq 2$, say that $e$ is contained in a temporal multi-edge.
Finally, we call an edge $e$ such that $\sigma(e) = \{v_i\}$, i.e. that connects node $v_i$ to itself, a \emph{loop} at $v_i$, and if $m(e) \geq 2$ or $w_{i,i,t} \geq 2$, we say that $e$ is contained in an (ordinary) \emph{multi-loop} or \emph{temporal multi-loop}, respectively.
Now, if an edge $e$ is neither a loop, nor contained in a temporal multi-edge, then we call $e$ a \emph{simple edge}, and we call a temporal graph \emph{simple} if it contains only simple edges, and no loops or temporal multi-edges.

We are now prepared to define the \emph{temporal degree} of a node and the \emph{temporal degree sequence} of a graph.
Given a node $v_i \in V$, we define its temporal degree as $d(v_i) = 2 m_{i,i} + \sum_{1 \leq j \neq i \leq n} m_{i,j}$, i.e. the number of incident edges over all timestamps but where we count loops twice as they occupy two possible endpoints for an edge.
Then, the temporal degree sequence lists the degrees of the nodes and specifies the number of available timestamps.
As our algorithms receive this sequence as input, it makes sense for us to consider the degree sequence independently of any graph, hence, we use the following definition:

\begin{definition}[Temporal Degree Sequence]
	A \emph{temporal degree sequence} $\mathbf{D} = (\mathbf{d}, T)$ of size $n$ consists of a vector $\mathbf{d}  \in \mathbb N^n_{> 0}$ and a a parameter $T \in \mathbb N_{>0}$.
	Given a temporal (multi-)graph $G = (V, E)$, we say that $G$ \emph{matches} the temporal degree sequence $\mathbf{D}$ if we have $d(v_i) = d_i$ for all temporal degrees of all nodes $v_i \in V$ and $\tau(e) \leq T$ for all timestamps of all edges $e \in E$.
	If there exists at least one \emph{simple} temporal graph $G$ which matches $\mathbf{D}$, then we call $\mathbf{D}$ \emph{realizable}.
	For a realizable temporal degree sequence $\mathbf{D}$ we write the set of all simple temporal graphs which match $\mathbf{D}$ as $\mathcal{G}(\mathbf{D})$.
\end{definition}

\noindent
We characterize a temporal degree sequence $\mathbf{D} = (\mathbf{d}, T)$ by the following properties.
\begin{equation}
	\nonumber
	\hfill \Delta = \max_{1 \leq i \leq n} d_i, \hfill M = \sum_{1 \leq i \leq n} d_i, \hfill M_2 = \sum_{1 \leq i \leq n} d_i (d_i - 1), \hfill
\end{equation}
i.e. $\Delta$ is the maximum temporal degree, $M$ the first moment and $M_2$ the second moment.
